Dilated Temporal Fully-Convolutional Network for Semantic Segmentation of Motion Capture Data

Semantic segmentation of motion capture sequences plays a key part in many data-driven motion synthesis frameworks. It is a preprocessing step in which long recordings of motion capture sequences are partitioned into smaller segments. Afterwards, additional methods like statistical modeling can be applied to each group of structurally-similar segments to learn an abstract motion manifold. The segmentation task however often remains a manual task, which increases the effort and cost of generating large-scale motion databases. We therefore propose an automatic framework for semantic segmentation of motion capture data using a dilated temporal fully-convolutional network. Our model outperforms a state-of-the-art model in action segmentation, as well as three networks for sequence modeling. We further show our model is robust against high noisy training labels.

==> sections/4_Results.tex <==
\section{Experimental Results}


\begin{figure}
	\centering
	\includegraphics[scale=.3]{images/prediction.png}
	\caption{top: 2D RGB image representation for a test sample, middle: ground truth pixel labels, bottom: predicted pixel labels.}
	\label{fig:prediction}
\end{figure}

Our motion capture dataset consists of  70 sequences with 4 main actions: \emph{walk}, \emph{pick}, \emph{place} and \emph{carry}. 
As an example, two of the semantic pixel labels for a walking motion are left-stance (poses in which left foot moves forward, colored green in  Figure~\ref{fig:mocap_rgb}, middle) and right-stance (poses in which right foot moves forward, colored red in  Figure~\ref{fig:mocap_rgb}, middle).
 In total we make use of 19 joints.
